Policy Learning with Competing Agents

Decision makers often aim to learn a treatment assignment policy under a capacity constraint on the number of agents that they can treat. When agents can respond strategically to such policies, competition arises, complicating estimation of the optimal policy. In this paper, we study capacity-constrained treatment assignment in the presence of such interference. We consider a dynamic model where the decision maker allocates treatments at each time step and heterogeneous agents myopically best respond to the previous treatment assignment policy. When the number of agents is large but finite, we show that the threshold for receiving treatment under a given policy converges to the policy's mean-field equilibrium threshold. Based on this result, we develop a consistent estimator for the policy gradient. In a semi-synthetic experiment with data from the National Education Longitudinal Study of 1988, we demonstrate that this estimator can be used for learning capacity-constrained policies in the presence of strategic behavior.

==> 15-extended-related-work.tex <==
% \rs{x What is the output of the ML model: A prediction, a classification, a treatment assignment, a ranking?

% x What is the objective function? Do they target prediction loss, policy loss, or something else? For a discussion of predictive vs policy loss in a non-strategic context, the following papers may be worth skimming:

%  Athey, Susan, and Stefan Wager. "Policy learning with observational data." *Econometrica* 89.1 (2021): 133-161.
%  Bertsimas, Dimitris, and Nathan Kallus. "From predictive to prescriptive analytics." *Management Science* 66.3 (2020): 1025-1044.
%   Kitagawa, Toru, and Aleksey Tetenov. "Who should be treated? empirical welfare maximization methods for treatment choice." *Econometrica* 86.2 (2018): 591-616.

% x How do the papers model counterfactuals? Do they use potential outcomes? Is there interference? Any strong parametric or structural assumptions?}

\begin{subsection}{Adversarial Classification.}
\cite{Dalvi04adversarialclassification}
\begin{enumerate}
    \item Due to the general intractability of finding Nash equilibria, they focus on a single-shot adversarial classification game where there is one move by each player. Use Naive Bayes classifier.
    \item Applications: spam detection, intrusion detection, fraud detection, surveillance, counter-terrorism (!?!), comparison shopping - merchants continually change their websites to avoid wrapping by shopbots, file sharing -- media companies try to detect illegal copying, web search- where  manipulations of pages/links are used to inflate ranking
    \item Output of ML model: a binary classification
    \item Objective function: expected utility -- which includes the aggregate costs of all correct and incorrect classifications (TP/FP/TN/FN) minus the cost of collecting information on different features (a decision maker may choose to not collect certain information on certain features).
    \item Assumptions: Assumes complete information -- the classifier and adversary know all the relevant parameters, adversary assumes that classifier is unaware of its presence, classifier assumes that adversary uses optimal strategy. Adversary/Classifier is perfectly rational.
    \item Interference: None.
\end{enumerate}
\end{subsection}

\begin{subsection}{Static Prediction Games for Adversarial Learning Problems.}
\cite{bruckner2012static}
\begin{enumerate}
    \item Emphasizes that although the goals of the learner and data generator may conflict, they are not entirely antagonistic (so minimax strategy is too pessimistic). Also, argues that Stackelberg games (where data generator has full knowledge of the model) is also too pessimistic. Instead, they study a setting where both players act simultaneously.
    \item Applications: computer/network security attacks are engineered with botnet and intrusion detection systems in mind, credit card defrauders adapt their transactions and behaviors to avoid getting flagged by credit card companies, senders of spam emails design message templates to pass through spam filters.
    \item Output of ML model: a binary classification
    \item Objective function: a weighted classification loss (the learner is more heavily penalized for misclassifying important emails than just generic (non-spam) emails)
    \item Modeling counterfactuals: No explicit mention of counterfactuals/potential outcomes.
    \item Assumptions: Complete information - both players know their opponent's cost function and action space. Also, players act simultaneously and are perfectly rational.
    \item Interference: None. In particular, they say (in the context of email spam filtering) that they ``study the competition between recipient and senders, not competition among senders" and they model ``all legitimate and abusive email senders as a single,
amalgamated player."
\end{enumerate}
\end{subsection}

\begin{subsection}{Strategic Classification.}
\cite{hardt2016strategic}
\begin{enumerate}
    \item Formalizes the problem of strategic classification and develops algorithms for learning classifiers that are robust to gaming. Classification is modeled as a sequential (Stackelberg) two-player game. 
    \item Develops a computationally-efficient learning algorithm for \textit{separable} cost functions and algorithms achieve classification error that approaches theoretical minimum.
    \item For general cost functions, designing an approximately optimal strategy-proof classifier for inverse-polynomial approximation is NP-hard.
    \item Applications: spam classification--argues that this is natural because spammers will game any automated attempt to identify them, stylized example of school admissions
    \item Output of ML model: a binary classification.
    \item Objective function: classification accuracy ($0-1$ loss)--they assume there is a \textit{target classifier} that maps agents' ``natural features" (they don't use this term) to the true classification label and compare the performance of the learned classifier on the observed features.
    \item Modeling counterfactuals: No explicit mention of counterfactuals/potential outcomes. Their objective function captures the classification accuracy when deploying different classifiers (but their notation sort of obscures the fact that deploying a particular classifier is an intervention...). They define \textit{strategic maximum}, which is the classification accuracy of the optimal classifier.
    \item Assumptions: Algorithm takes as input the agent's cost function $c$ and data consisting of natural features and true label pairs. (In contrast, in our setting the decision maker doesn't know agents' cost function and doesn't observe any natural features/perfectly labeled data--instead, the decision maker observes a loss after deploying a model.) The learner has (almost) full knowledge of the agents’ utility functions; in particular, it is assumed that the learner has access to the “true” distribution of agent features (before manipulation), and that the costs experienced by the agents for manipulating their data are the same for all agents and known to the learner.
    \item Interference: None.
\end{enumerate}
\end{subsection}



\begin{subsection}{The Social Cost of Strategic Classification.}
\cite{milli2019social}
Similar to \cite{hardt2016strategic}.
\begin{enumerate}
    \item Studies the tension between accuracy of the institution and impact on the individuals being classified when institutions deploy classifiers that are more "strategy robust"-- argues that honest individuals may need to invest more to be classified correctly.
    \item Stackelberg solution maximizes institutional accuracy at the expense of maximal social burden.
    \item Output of ML Model: A binary classification.
    \item Objective function: Classification accuracy (after individuals game).
    \item Modeling counterfactuals: Considers the classification accuracy, social burden under different classifiers. Similar to \cite{hardt2016strategic}, notation obscures the fact that observed covariates are a function of the deployed classifier.
    \item Assumptions: Agents have outcome monotonic costs which have two properties: 1) increasing one's outcome requires monotonically increasing amounts of work, 2) it is zero cost to worsen one's outcome.
    \item Interference: None. Specifically, they say "since individuals game optimally, when an individual changes her features in response to the classifier $f$ she has no incentive to move to a point with likelihood higher than [the threshold of the classifier]."
\end{enumerate}
\end{subsection}

\begin{subsection}{Gaming helps! Learning from strategic interactions in natural dynamics.}
\cite{bechavod2021gaming}
\begin{enumerate}
    \item Strategic manipulation may help the learner recover meaningful features, the features that when changed, affect the true label. Non-meaningful variables do not affect the true label but can potentially be used to obtain better outcomes with respect to the posted model without improving true labels.
    \item Online learning with no strategic response has no ability to distinguish non-meaningful variables from meaningful ones when the two are correlated.
    \item They assume that there is a true latent regression parameter $\beta^{*}$ that \textit{generates} an agent's label as a function of his unmodified feature vector. The agents' gamed features $\overline{x}_{t}$. The decision maker observes $\overline{y}_{t} = \beta^{*} \overline{x}_{t} + \epsilon_{t}$ at the end of each round.
    \item Applications: credit assessment, school admissions.
    \item Output of ML Model: A continuous-valued score.
    \item Assumptions: There is some true regression parameter $\beta^{*}$ that generates the true labels. Agents best respond perfectly. Decision maker does not true features or cost function but sees the agent's realized label after feature modification.
    \item Interference: None
\end{enumerate}
\end{subsection}

\begin{subsection}{Alternative Microfoundations for Strategic Classification.}
\cite{jagadeesan2021alternative}
\begin{enumerate}
    \item Proposes noisy response model to address issues that arise when combining the standard microfoundations of rational agents with statistical decision theory. Issues include discontinuities, lack of robustness to agents who are not perfectly strategic, maximization of social burden.
    \item Assume that each agent best responds to a noisy version of the model parameters-- $\theta + \zeta$ where $\zeta$ is sampled from some zero-mean distribution.
    \item Output of ML model: a binary classification. The ML model in this case is just 1-dimensional $\mathbb{I}(x \geq \theta)$, so the model parameters are just the threshold.
    \item Objective function: Classification accuracy (0-1 loss)
    \item Assumptions: Noisy response model that they propose captures the idea of an imperfect agent, who has imperfect control over actions/opaque access to the classifier/interpretability issues.
    \item Modeling counterfactuals: Classification accuracy and social burden obtained under different classifiers.
    \item Interference: None.
\end{enumerate}
\end{subsection}

\begin{subsection}{Strategic Classification from Revealed Preferences.}
\cite{dong2018strategic}
\begin{enumerate}
\item Focuses on online setting of strategic classification-- learner does not know the utility functions of the agents: neither their true features $x$, nor the cost they experience for manipulation (which can now differ for each agent). They model the learning process as an iterative, online procedure.
\item Learner gets to observe true label at the end of the round, but never gets to see the true features or the cost function for manipulation (they may be adversarially chosen, might not come from a distribution).
\item Instead of assuming that all agents are strategic, only agents with true negative classification are strategic.
    \item Output of ML model: The goal is binary classification but TBH the output of the ML model is actually a score that gets plugged into the hinge loss or logistic loss.
    \item Objective function: Stackelberg regret - comparing the average loss of the learner to the loss she could have experienced with the best fixed classifier in hindsight, taking into account that the agents would have best-responded differently had she
used a different classifier. Focuses on two classification loss functions.
    \item Assumptions: Only negatively classified agents are strategic. Learner does not know agents' cost functions or true features. Agents play exact best responses.
    \item Modeling counterfactuals: Not really?
    \item Interference: None
\end{enumerate}
\end{subsection}

\begin{subsection}{Improving Information From Manipulable Data}

\begin{enumerate}
    \item Naive designer uses a static decision rule $Y(x) = \beta x + \beta_{0}$. A more sophisticated designer may gather new data, re-estimate relationship between observable features and loss, which yields the fixed point allocation rule. The optimal rule is the Stackelberg solution, where $\beta$ to minimize welfare loss with knowledge of that agents will game.
    \item Stackelberg solution is "flatter" has smaller $\beta$ than fixed point rule.
    \item At fixed points, misallocation loss is 0 but there is positive information loss. Information loss increases as $\beta$ increases. The optimal policy (Stackelberg solution) has $\beta < \beta_{\text{FP}}$.
    \item Applications: Price discrimination, search engine optimization, credit scoring, product reviews.
    \item Output of ML Model: A continuous-valued allocation.
    \item Objective function: Welfare loss-- MSE of the allocation compared to the natural ability of the agents (decomposition into misallocation loss  and information loss). Information loss results from incorrectly estimating $\eta$ from $x$ and misallocation loss results from giving the wrong allocation given the estimated $\eta$. Designer aims to maximize allocation accuracy when accounting for manipulation.
    \item Modeling counterfactuals: Welfare loss under different models.
    \item Assumptions: Agents have type $(\eta, \gamma)$ where $\eta$ is natural ability and $\gamma$ is gaming ability. Decision maker observes $x$, covariates after manipulation. The agent optimizes a cost function depending on their allocation (which depends on $\beta$) and their type $(\eta, \gamma)$ and there's a closed form for the best response. Decision maker does not know agents' private type or cost function.
    \item Interference: None.
\end{enumerate}

\end{subsection}


\begin{subsection}{Learning to Personalize Treatments When Agents are Strategic}
\cite{munro2020learning}

\begin{enumerate}
    \item Provides a general model of how policy targeting induces endogeneity in observed individual-level data and why new methods for developing treatment allocation rules are needed. Argues that impact of strategic responses on decision maker's loss needs to be accounted for.
    \item Uses same method as \cite{wager2021experimenting} to learn optimal model in the strategic setting.
    \item Applications: Heterogeneous pricing, individualized credit offers, targeted social programs, predicting quality of content on social media platforms using click-through rates.
    \item Output of ML Model: A continuous treatment.
    \item Objective function: Policy loss that depends on the treatment that individuals' receive and their outcomes.
    \item Modeling counterfactuals: Uses potential outcomes-- ML model outputs treatments, individuals' post-treatment outcomes are observed (which may depend on the treatment received and private type).
    \item Parametric/structural assumptions: Does not make parametric assumptions on individual strategic behavior.
    \item Interference: None.
\end{enumerate}
\end{subsection}


\begin{subsection}{Strategic Ranking.}
\cite{liu2021strategic}
\begin{enumerate}
    \item Studies tradeoff between applicant, school, and societal utility in the setting where agents are strategic and agents' reward depends on relative position in the ranking. 
    \item By reducing the degree of randomization in the admission policy, private utility of the school is increased at the expense of applicant welfare. The authors comment that unfortunately-- the school has no incentive to use a more randomized classifier.
    \item Applications: College admissions, job hiring.
    \item Output of ML Model: There isn't really an ML model because there's no learning in this paper. The agents' effort and pre-effort skill level are inputs to a function that produces a score for each applicant. The scores are used to generate post-effort ranking. In the $d$-dimensional setting (where agents have $m$ latent skills), the applicants choose the amount of effort $e_{i}$ they want to invest in each skill $i$, yielding $m$ post-effort scores. The school announces weights $\alpha \in \Delta_{m}$ ($m$-dimensional simplex) for each skill in the admission decision and ranks applicants based on their combined weighted score.
    \item Objective function: There are 2 -- the more relevant one is the school's utility function. Societal utility -- which is the mean post-effort score (society prefers the entire applicant population to achieve higher scores), School's private utility -- expected score of admitted applicants.
    \item Modeling counterfactuals: They consider the effect of different ranking reward functions $\lambda$, which take in an applicants' post-effort rank.
    \item Assumptions: Agents are homogeneous in gaming ability, which gives rise to \textit{rank preservation} (post-effort ranks are identical to pre-effort ranks). Each agent has an unobserved skill level (yields a pre-effort rank), applicants choose an effort level (based on the ranking reward design). Investment in effort yields a post-effort score (yields post-effort rank when compared to other applicants).
    \item Interference: The term interference is not explicitly used but considers the effect of \textit{competition} among individuals due to the constrained allocation setting. Competition between applicants affects their effort and their comparative performance/position in the ranking.
\end{enumerate}
\end{subsection}


\begin{subsection}{Muddled Information}
\cite{frankel2019muddled}

\begin{enumerate}
    \item Muddled information arises because there is unobservable heterogeneity across agents in their ability to game
    \item The agent prefers higher market beliefs on their quality, higher beliefs are more valuable when stakes are higher.
    \item Identifies relationship between the signaling costs of cross-types --pairs in which one has higher natural action but lower gaming ability than another
    \item Key assumption: At low levels of signaling (low stakes), differences in marginal cost are driven by differences in natural action. At higher levels of signaling , they depend more on differences in gaming ability.
    \item Observation that when stakes of signaling increase/costs of signaling decrease, the muddled information reveals more about agent's gaming ability than natural action.
    \item Applications: Search engine optimization, credit scoring, college admissions/SAT scores
    \item Output of ML Model: No ML model. Agent cares about getting higher market beliefs on their quality
    \item Objective function: N/A
    \item Modeling counterfactuals: N/A
    \item Parametric/structural assumptions: Similar to our setting agents are heterogeneous in gaming ability and natural ability. Agent chooses an action $a$. Consider cross-types natural $(\overline{\eta}, \underline{\gamma})$ and gamer $(\underline{\eta}, \overline{\gamma})$. Cost function is designed so that at higher actions, the marginal cost to gamer is less than marginal cost to natural, and at lower actions, the marginal cost to natural is less than marginal cost to gamer. Order-reversing action is where this reverses. 
    \item Interference: None
\end{enumerate}
\end{subsection}

% \begin{subsection}{Inferring welfare maximizing treatment assignment under budget constraints.}

% \end{subsection}

\begin{subsection}{Other works}
\begin{enumerate}
    \item Marketplace interference \cite{blake2014marketplace} \cite{heckman1998general} \cite{wager2021experimenting} \cite{munro2021treatment}.
    \item Causal inference and interference \cite{hu2021average}.
    \item Decision-making with budget constraint \cite{bhattacharya2012inferring}.
    \item Performative prediction \cite{izzo2021learn}, \cite{miller2021outside}, \cite{perdomo2020performative}
    \item Treatment allocation rules \cite{manski2004statistical}
\end{enumerate}
The literature on mechanism design for tournament-type settings may also be relevant.
For a starting point and references, there's:
``Targeting in Tournaments with Dynamic Incentives'' by Banchio and Munro.

\end{subsection}




    %for any pair of cross types, the ratio of marginal costs of the high natural action type to the high gaming ability type is increasing in the action -- as more gaming occurs, cost differences are driven more by differences in gaming ability
    % \item Showing agents' actions to additional observers can worsen information for existing observers (bc stakes are higher)

    % \item Agents are heterogenous on two dimensions - natural action and gaming ability. As incentives to take higher actions increases, more information is revealed about gaming ability  and less about natural actions. 
    % \item As incentives to take higher actions increase, due to higher stakes or more easily manipulated signaling technology, more information is revealed about gaming ability, and less about natural actions.
% \begin{subsection}{Muddled information.}
% \cite{frankel2019muddled}
% \begin{itemize}
%     \item As incentives to take higher actions increase, due to higher stakes or more easily manipulated signaling technology, more information is revealed about gaming ability, and less about natural actions.
%     % \item Spence-Mirrlees single-crossing condition - ensure existence of separating equilibria, so that only cost of gaming is through a costly increase in effort
%     % \item homogeneity of natural actions OR gaming ability, lead to full separation (...similarly, we can say that there exists a single fixed point when agents are homogenous along one of these axes)
%     % \item at low levels of signaling, differences in marginal costs are driven by differences in natural actions. at high levels of signaling, differences are driven by differences in gaming ability.
%     % \item Conjecture -- when threshold is very high, people who win have high natural ability (bc no one can game), when threshold is sort of high, people who win have high gaming ability. when threshold is moderate, people who win have high natural ability and high gaming ability
%     \item Muddled information arrises because there is unobservable heterogeneity across agents in their ability to game
%     \item Main contribution-- developing the comparative statics of market information when it is muddled, uncovering the general forces underlying these comparative statics.
%     \item $\theta = (\eta, \gamma) \sim F$ with compact support $\Theta \subset \mathbb{R} \times \mathbb{R}_{++}.$
%     \item $\eta$ is the intrinsic ideal point - highest action she can take at minimum cost.
%     \item $\gamma$- cost of increasing action above the natural level.
%     % \item Assumptions: 
%     % \begin{enumerate}
%     %     \item natural action $a = \eta$ is an agent's highest cost-minimizing action, with cost normalized to zero
%     %     \item agent can costlessly take actions below her natural actions (free downward deviations)--this is not true in our model, deviating from $\eta$ has above and below has the same cost.
%     %     \item marginal cost is $0$ at natural action
%     %     \item increasing convex cost to take higher actions.
%     %     \item marginal cost of increasing one's action is lower for agents with either higher natural actions or higher gaming ability.
%     %     \item cost function satisfies decreasing differences (i.e. single-crossing property): if $\underline{a} < \bar{a}$ and $\underline{\theta} < \bar{\theta}$ in component-wise order, then 
%     %     \[ C(\bar{a}, \underline{\theta}) - C(\underline{a}, \underline{\theta}) \geq C(\bar{a}, \bar{\theta}) - C(\underline{a}, \bar{\theta}).\]
%     %     \item For any $\underline{\eta} < \bar{\eta}$ and $\underline{\gamma} < \bar{\gamma}$, $C_{a}(\cdot, \bar{\eta}, \underline{\gamma})/C_{a}(\cdot, \underline{\eta}, \overline{\gamma})$ is strictly increasing on $[\bar{\eta}, \infty)$, there exists an order-reversing action $a^{or} > \bar{\eta}$ s.t. $C_{a}(a^{or}, \bar{\eta}, \underline{\gamma}) = C_{a}(a^{or}, \underline{a}, \bar{\gamma}).$
%     % \end{enumerate}
%     % \item Equilibria is separating if it fully reveals the agent's private information on the dimension of interest, an equilibrium is pooling if it reveals no information on the dimension of interest, an equilibrium is partially-pooling if it is neither separating nor pooling.
%     % \item equivalent equilibria - share the same mapping from types to distributions over the posterior belief and the same mapping from types to distributions over signalling costs.
%     % \item What does on-path actions means?
%     % \item signaling games - typically having a pooling equilibrium, equilibrium beliefs are monotonic in actions.
%     % \item results don't change even if downward deviations were made costly (so our costs should be equivalent...)

%     % \item any equilibrium induces a probability distribution over $\beta_{\tau}$. A distribution of beliefs is more informative than another if the former is a mean-preserving spread of the latter.
%     % \item partial ordering of equilibria...there is higher allocative efficiency when beliefs are more informative
% \end{itemize}


==> 16-relevance-eaamo.tex <==
% A 200-250 word description summarizing the submission and its relevance to the conference

We study capacity-constrained treatment assignment in the presence of strategic behavior. Decision makers often aim to map observed individual characteristics to treatment assignments. However, when human agents being considered for the treatment have knowledge of the assignment policy, the observed data depends on the deployed policy. In the context of college admissions, strategic behavior arises while the decision maker also has a capacity constraint on the number of agents they can treat. For example, students may enroll in test preparation services and take advanced courses to improve their chances of getting accepted to college, while college can only accept a small fraction of the applicant pool. Our model illustrates that the combination of capacity constraints and strategic behavior yields competition, which impacts the overall effect of the policy. An assumption that we center in this work is that agents are heterogeneous in their ability to respond to the treatment assignment policy. This captures the observation that in college admissions, different students may have different levels of resources at their disposal to invest in changing their behavior to respond to the admissions policy. Our work is relevant to EAAMO because our model can be used to study the capacity-constrained allocation of educational resources in the presence of heterogeneous strategic behavior. Our model is based on previous work in economics and game theory, and our proposed method for learning policies in this model draws on statistics and machine learning.

==> archive.tex <==
% \begin{lemm}
% \label{lemm:concentration_quantiles}
% Let $P$ be a distribution function with positive density $p$ on $\mathbb{R}$ and let $P^{n}$ be its corresponding empirical distribution. Suppose $B$ is a large constant such that $|q(P)| < B$. Let
% \begin{align*}
%     D&:= \inf_{r \in [-2B, 2B]} p(r) \\
%     C_{n} &:= P(|q(P) - q(P^{n})| < B).
% \end{align*}
% For $\epsilon > 0$ and $n > 0$ 
% \[ P(|q(P) - q(P^{n})| < \epsilon ) \geq (1 - 2e^{-2nD^{2} \epsilon^{2}}) \cdot C_{n}.\]
%  \hyperref[subsec:concentration_quantiles]{Proof in Appendix \ref{subsec:concentration_quantiles}}.
% \end{lemm}


% \begin{subsection}{Proof of Lemma \ref{lemm:quantile_bound}}
% \label{subsec:quantile_bound}
% %As a result, the probability of event $B$ can be lower bounded by the probability of event $A$.

% Since $P$ and $\tilde{P}$ are both surjective functions, there exist $r_{1}, r_{2}$ in $\mathcal{X}$ such that 
% $P(r_{1}) = q$ and $\tilde{P}(r_{2}) = q.$ In other words, $r_{1} = q(P)$ and $r_{2} = q(\tilde{P})$. Since $|q(P)| < B$ and $|q(\tilde{P}) - q(P)| < B$, then $|q(\tilde{P})| < 2B$. Thus, we have that $r_{1}, r_{2} \in [-2B, 2B].$ We have that
% \begin{align}
%     |P(r_{2}) - \tilde{P}(r_{2})| &= |P(r_{2}) - P(r_{1})| \label{eq:q1} \\
%     &= |p(\lambda r_{1} + (1- \lambda) r_{2}) (r_{2} - r_{1}) | \text{ where }  \lambda \in [0, 1]  \label{eq:q2}\\
%     &= |p(\lambda r_{1} + (1- \lambda) r_{2})| |r_{2} - r_{1} | \label{eq:q3} \\
%     &\geq \inf_{ \lambda \in [0, 1]} |p(\lambda r_{1} + (1- \lambda) r_{2})|  |r_{2} - r_{1} | \label{eq:q4} \\
%     &\geq \inf_{r \in [-2B, 2B]} |p(r)| \cdot |r_{2} - r_{1}| \label{eq:q5} \\
%     &= D \cdot |r_{2} - r_{1}|. \label{eq:q6}
% \end{align}
% \eqref{eq:q1} follows from $q = P(r_{1}) = \tilde{P}(r_{2}).$ \eqref{eq:q2} is an application of the Mean Value Theorem. \eqref{eq:q3} holds because $p(\lambda r_{1} + (1- \lambda) r_{2})$. \eqref{eq:q5} holds because $r_{1}, r_{2} \in [-2B, 2B]$. \eqref{eq:q6} follows from the definition of $D$. As a result, we have that
% \begin{align*}
%     |q(P) - q(\tilde{P})| &\leq \frac{1}{D} |P(r_{2}) - \tilde{P}(r_{2})| \\
%     &\leq \frac{1}{D} \sup_{r \in \mathbb{R}} |P(r) - \tilde{P}(r)|.
% \end{align*}

% \end{subsection}

% \begin{subsection}{Proof of Lemma \ref{lemm:concentration_quantiles}}
% \label{subsec:concentration_quantiles}
% First, we note that if the event $\{|q(P^{n}) - q(P)| > B\}$ occurs then we cannot have that the event $\{|q(P^{n}) - q(P)| < \epsilon\}$ occurs. In addition, if the event $\{|q(P^{n}) - q(P)| < B\}$ occurs then the event $\{|q(P^{n}) - q(P)| < \epsilon\}$ may also occur.

% Suppose $\{|q(P^{n}) - q(P)| < B\}$ occurs. Then we have that $|q(P^{n})| \leq 2B$. By assumption, we have that $|q(P)| \leq B \leq 2B.$ So, on this event we have both $|q(P)|, |q(P^{n})| \leq 2B$. We can apply Lemma \ref{lemm:quantile_bound} to see that on this event, we have that
% \[ |q(P) - q(P^{n})| \leq \frac{1}{D} \cdot \sup_{r \in \mathbb{R}} |P(r) - P^{n}(r)|.\]
% We observe that if $\sup_{r \in \mathbb{R}} |P(r) - P^{n}(r)| \leq D\epsilon$, then $|q(P) - q(P^{n})| \leq \epsilon.$
% Thus, by Theorem \ref{theo:dkw}, we have that
% \begin{align*}
%     &P(|q(P) - q(P^{n})| \leq \epsilon ) \\
%     &= P(|q(P) - q(P^{n})| \leq \epsilon, |q(P) - q(P^{n})| \leq B ) + P(|q(P) - q(P^{n})| \leq \epsilon, |q(P) - q(P^{n})| > B ) \\
%     &= P(|q(P) - q(P^{n})| \leq \epsilon \mid |q(P) - q(P^{n})| \leq B ) P(|q(P) - q(P^{n})| \leq B) \\
%     &= C_{n} \cdot P(|q(P) - q(P^{n})| \leq \epsilon \mid |q(P) - q(P^{n})| \leq B ) \\
%     &\geq C_{n} \cdot P( \sup_{r \in \mathbb{R}} |P(r) - P^{n}(r)| \leq D\epsilon \mid |q(P) - q(P^{n})| \leq B ) \\
%     &\geq (1 - 2e^{-2nD^{2} \epsilon^{2}}) \cdot C_{n},\\
% \end{align*}
% where the last line follows from Lemma \ref{lemm:bound_q}.
% \end{subsection}


% \begin{subsection}{Proof of Lemma \ref{lemm:bound_q}}
% \label{subsec:bound_q}
% Recall that $\bfepsilon \sim N(0, \sigma^{2}I_{d}).$ Let $q_{\bfepsilon}$ denote the $q$-th quantile of $\bfbeta^{T}\bfepsilon.$ We can develop bounds on $q(P_{\bfbeta, s})$ by considering two new distributions. Let $P^{l}_{\bfbeta, s}$ be the distribution over $\inf_{\nu \in \text{supp}(F)} \bfbeta^{T}\bfx(\bfbeta, s, \nu).$ Let $P^{u}_{\bfbeta, s}$ be the distribution over $\sup_{\nu \in \text{supp}(F)} \bfbeta^{T}\bfx(\bfbeta,s, \nu).$ We realize that 
% \begin{align}
%     q(P^{u}_{\bfbeta, s}) &= \sup_{\nu \in \text{supp}(F)} \bfbeta^{T} \bfx^{*}(\bfbeta,s, \nu) + q_{\epsilon} \label{eq:upper}, \\
%     q(P^{l}_{\bfbeta, s}) &= \inf_{\nu \in \text{supp}(F)} \bfbeta^{T} \bfx^{*}(\bfbeta,s, \nu) + q_{\epsilon} \label{eq:lower}.
% \end{align}
% It is clear that
% \[ q(P^{l}_{\bfbeta, s}) \leq q(P_{\bfbeta, s}) \leq q(P^{u}_{\bfbeta, s}).\]
% Under Assumption \ref{assumption:finite_types}, there are some $\nu^{u}, \nu^{l}$ for which the $\sup$ in \eqref{eq:upper} and $\inf$ in \eqref{eq:lower} are achieved, respectively. By Lemma \ref{lemm:shape_br}, $s \mapsto \bfbeta^{T}\bfx^{*}(\bfbeta, s, \nu^{u})$ is maximized at some point $s^{*}_{\nu^{u}}.$ So,
% \[ \sup_{s \in \mathbb{R}} q(P^{u}_{\bfbeta, s}) = \bfbeta^{T}\bfx^{*}(\bfbeta, s^{*}_{\nu^{u}}, \nu^{u}) + q_{\epsilon}.\]
% By Lemma \ref{lemm:shape_br} and Lemma \ref{lemm:limits_br}, we have that $\inf_{s \in \mathbb{R}} \bfbeta^{T}\bfx^{*}(\bfbeta,s, \nu^{l}) = \bfbeta^{T}\bfeta^{l}$, where $\nu^{l}= (\bfeta^{l}, \bfgamma^{l}) + q_{\epsilon}$. So,
% \[ \inf_{s \in \mathbb{R}} q(P^{l}_{\bfbeta, s}) = \bfbeta^{T}\bfeta^{l}.\]
% Let $B = \max\{|\bfbeta^{T}\bfeta^{l} + q_{\epsilon}|, |\bfbeta^{T}\bfx^{*}(\bfbeta, s_{\nu^{u}}^{*}, \nu^{u})  + q_{\epsilon}|\}.$ Finally, we conclude that $q(P_{\bfbeta, s}) \leq B$ for all $s \in \mathbb{R}.$
% \end{subsection}

% We state lemmas that will be used in our subsequent results.

% \begin{lemm}
% \label{lemm:bound_q}
% Fix $\bfbeta \in \mathcal{B}.$ Under Assumptions \ref{assumption:strong_convexity}, \ref{assumption:finite_types}, \ref{assumption:br_interior}, there exists $B > 0$ such that $|q(P_{\bfbeta, s})| \leq B$ for all $s \in \mathbb{R}.$
% \hyperref[subsec:bound_q]{Proof in Appendix \ref{subsec:bound_q}}.
% \end{lemm}


% \begin{lemm}
% \label{lemm:almost_sure_quantiles}
% \rs{TODO almost sure convergence of empirical quantiles to sample quantiles}
% \end{lemm}


% \begin{lemm}
% \label{lemm:quantile_bound}
% Let $P$ be a distribution function with positive density $p$ on $\mathbb{R}$. Let $\tilde{P}$ be a distribution function on $\mathbb{R}.$ Suppose $B$ is an upper bound on $|q(P)|,$ $|q(P) - q(\tilde{P})|$. Let 
% \[ D:= \inf_{r \in [-2B, 2B]} p(r).\]
% Then,
% \[ |q(P) - q(\tilde{P})| \leq \frac{1}{D} \sup_{r \in \mathbb{R}} |P(r) - \tilde{P}(r)|.\]

% % Let $D >0$ be a lower bound on the derivative of $P$. Then,
% % \begin{equation} 
% % \label{eq:quantile_bound}
% % |q(P) - q(\tilde{P})| \leq \frac{1}{D} \sup_{r \in \mathcal{X}} |P(x) - \tilde{P}(x)|. 
% % \end{equation}
% \hyperref[subsec:quantile_bound]{Proof in Appendix \ref{subsec:quantile_bound}}.
% \end{lemm}

% First, we note that the constant $B>0$ such that $|q(P_{\bfbeta, s})| \leq B$ for all $s \in \mathbb{R}$ exists by Lemma \ref{lemm:bound_q}.

\rs{fix this there should be a simpler proof}
% We define a distribution that will be used to demonstrate the existence of $s_{l}$ and $s_{h}.$ Let $P$ be the distribution over $\bfbeta^{T}(\bfeta + \bfepsilon)$ where $\nu=(\bfeta, \bfgamma) \sim F$ and $\bfepsilon \sim N(0, \sigma^{2}I_{d}).$ Let $q(P)$ be the $q$-th quantile of $P$.

First, we show that there exists $s_{l}$ such that $g(s_{l}) < 0$. By Lemma \ref{lemm:limits_br}, for every agent type $\nu=(\bfeta, \bfgamma)$, there is $S_{l, \nu} \in \mathbb{R}$ so that for all $s \leq S_{l, \nu},$ we have that
\[ |\bfbeta^{T}\bfx^{*}(\bfbeta, s, \nu) - \bfbeta^{T}\bfeta| < \delta.\]
Let
\[ S_{l, 1} = \inf_{\nu \in \text{supp}(F)} S_{l, \nu}.\]
Also, by Assumption \ref{assumption:finite_types}, $S_{l, 1} > -\infty.$ When $s \leq S_{l, 1}$, we have that 
\[ q(P) - \delta \leq q(P_{\bfbeta, s}) \leq q(P) + \delta.\]
Let $S_{l, 2} = q(P) - \delta$ . Let $s_{l} < \min(S_{l, 1}, S_{l, 2}).$ Thus, we have that
\begin{align*}
    g(s_{l}) &= s_{l} - q(P_{\bfbeta, s_{l}}) \\
    &\leq s_{l} - q(P) + \delta \\
    &< (q(P) - \delta) - q(P) + \delta \\
    &= 0.
\end{align*}
The second line follows because $s_{l} < S_{l, 1},$ so $q(P_{\bfbeta, s_{l}}) \geq q(P) - \delta$. The third line follows because $s_{l} < S_{l, 2}$, so $s_{l} \leq q(P) - \delta.$

Second, we show that there exists $s_{h}$ such that $g(s_{h}) > 0$ and $s_{h} > s_{l}$. By Lemma \ref{lemm:limits_br}, we note that for every agent type $\nu=(\bfeta, \bfgamma),$ there is $S_{h, \nu} \in \mathbb{R}$, so that for $s \geq S_{h, \nu}$
\[|\bfbeta^{T}\bfx^{*}(\bfbeta, s, \nu) - \bfbeta^{T}\bfeta | < \delta.\]
Let \[S_{h, 1} = \sup_{\nu \in \text{supp}(F)}S_{h, \nu}.\] 
In addition, by Assumption \ref{assumption:finite_types}, $S_{h, 1} < \infty$. Then, when $s \geq S_{h, 1}$, we have that 
\[ q(P) - \delta \leq q(P_{\bfbeta, s}) \leq q(P) + \delta.\]
Let $S_{h, 2} = q(P) + \delta$. Let $s_{h} > \max(S_{h, 1}, S_{h, 2}).$ We note that 
\begin{align*}
    g(s_{h}) &= s_{h} - q(P_{\bfbeta, s_{h}}) \\
    &\geq s_{h} - q(P) - \delta \\
    &> (q(P) +\delta) - q(P) - \delta\\
    &= 0.
\end{align*}
Finally, we show that $s_{h} > s_{l}.$ From Lemma \ref{lemm:shape_br}, we have that $S_{h, \nu} \geq s^{*}_{\nu}$ and $S_{l, \nu} \leq s^{*}_{\nu}$ for every $\nu$, where $s^{*}_{\nu}$ maximizes $\omega(s; \bfbeta, \nu).$. So,
\[ S_{h, 1} \geq \sup_{\nu \in \text{supp}(F)} s^{*}_{\nu},\] while
\[ S_{l, 1} \leq \inf_{\nu \in \text{supp}(F)} s^{*}_{\nu}.\]
This yields
\begin{align*}
    s_{h} &> S_{h, 1} \\
    &\geq \sup_{\nu \in \text{supp}(F)} s^{*}_{\nu} \\
    &\geq \inf_{\nu \in \text{supp}(F)} s^{*}_{\nu} \\
    &\geq S_{l, 1} \\
    &> s_{l}.
\end{align*}



% We combine the results of Theorems \ref{theo:direct_effect} and \ref{theo:indirect_effect}. Let $\{b_{\text{ME}, n} \}$ denote the sequence $\{b_{n}\}$ where $b_{n} \rightarrow 0$ so that \[\hat{\tau}_{\text{ME}, n}^{t_{n}}(\bfbeta) \xrightarrow{p} \tau_{\text{ME}}(\bfbeta).\] Let $\{b_{\text{EE}, n} \}$ denote the sequence $\{b_{n}\}$ where $b_{n} \rightarrow 0$ so that \[\hat{\tau}_{\text{EE}, n}^{t_{n}}(\bfbeta) \xrightarrow{p} \tau_{\text{EE}}(\bfbeta).\]
% We can show that there exists a sequence $\{b_{\text{PE}, n}\}$ where $b_{\text{PE}, n} \rightarrow 0$ so that \[\hat{\tau}_{\text{PE}, n}^{t_{n}}(\bfbeta) \xrightarrow{p}  \tau_{\text{PE}}(\bfbeta).\]

% Let $b_{\text{PE}, n} = \max(b_{\text{ME}, n}, b_{\text{EE}, n})$. First, we verify that $b_{\text{PE}, n} \rightarrow 0.$ Since $b_{\text{ME}, n} \rightarrow 0$, there exists $N_{1} \in \mathbb{N}$ such that $|b_{\text{ME}, n}| < \epsilon$ for $n \geq N_{1}.$ Similarly, there exists $N_{2} \in \mathbb{N}$ such that  $|b_{\text{EE}, n}| < \epsilon$ for $n \geq N_{2}.$ For $n \geq \max(N_{1}, N_{2}),$ we have that $|b_{\text{PE}, n}| < \epsilon.$ So, $b_{\text{PE}, n} \rightarrow 0.$

% Now, we show that $\hat{\tau}_{\text{PE}, n}^{t_{n}}(\bfbeta) \xrightarrow{p} \tau_{\text{PE}}(\bfbeta)$ for this sequence of perturbations.
% Let $\hat{\tilde{\tau}}_{\text{ME}, n}^{t_{n}}(\bfbeta)$ be a model effect estimator with $\{b_{n}\} = \{ b_{\text{PE}, n}\}$. Similarly, let $\hat{\tilde{\tau}}_{\text{EE}, n}^{t_{n}}(\bfbeta)$ be a equilibrium effect estimator with $\{b_{n}\} = \{ b_{\text{PE}, n}\}$. We observe that
% \begin{align*}
%     |\hat{\tau}_{\text{PE}, n}^{t_{n}}(\bfbeta)- \tau_{\text{PE}}(\bfbeta)| &=
%     |\hat{\tilde{\tau}}_{\text{ME}, n}^{t_{n}}(\bfbeta) + \hat{\tilde{\tau}}_{\text{EE}, n}^{t_{n}}(\bfbeta) - \tau_{\text{ME}}(\bfbeta) - \tau_{\text{EE}}(\bfbeta) | \\
%     &\leq |\hat{\tilde{\tau}}_{\text{ME}, n}^{t_{n}}(\bfbeta) - \tau_{\text{ME}}(\bfbeta)| + |\hat{\tilde{\tau}}_{\text{EE}, n}^{t_{n}}(\bfbeta) - \tau_{\text{EE}}(\bfbeta) |, 
% \end{align*}
% so to show prove convergence in probability of the policy effect estimator it is sufficient to show that the terms on the right side of the above equation are $o_{p}(1).$

% We certainly have that $|\hat{\tau}_{\text{ME}, n}^{t_{n}}(\bfbeta) - \tau_{\text{ME}}(\bfbeta)| = o_{p}(1)$. So, for $n \geq n_{1}(\epsilon, \delta)$, we have that
% \[ P(|\hat{\tau}_{\text{ME}, n}^{t_{n}}(\bfbeta) - \tau_{\text{ME}}(\bfbeta)| \geq \epsilon ) \leq \delta.\]
% Let $b_{1}(\epsilon, \delta) = b_{\text{ME}, n_{1}(\epsilon, \delta)}$. Since $b_{\text{PE}, n} \rightarrow 0$, $|b_{\text{PE}, n}| < b_{1}(\epsilon, \delta)$ for $n \geq \tilde{n}_{1}(\epsilon, \delta).$
% By the definition of $b_{\text{PE, n}}$, we must have that $n_{1}(\epsilon, \delta) \leq \tilde{n}_{1}(\epsilon, \delta).$ So, when 
% $n \geq \tilde{n}_{1}(\epsilon, \delta),$ we have that 
% \[ P(|\hat{\tilde{\tau}}_{\text{ME}, n}^{t_{n}}(\bfbeta) - \tau_{\text{ME}}(\bfbeta)| \geq \epsilon ).\]
% A
% Similarly, for $n \geq n_{2}(\epsilon, \delta)$, we have that
% \[ P(|\hat{\tau}_{\text{ME}, n}^{t_{n}}(\bfbeta) - \tau_{\text{ME}}(\bfbeta)| \geq \epsilon ) \leq \delta.\]


% \begin{align*}
%     \Gamma_{\ell, \bfbeta}^{k} &=  \argmin_{\Gamma \in \mathbb{R}^{d}} \EE[\epsilon \sim G, \nu \sim F, \bfzeta \sim R^{d}] {(\ell(\pi_{\epsilon}(g(\bfbeta + k\bfzeta, s, \nu); \bfbeta, q(P_{\bfbeta + k\bfzeta, s})), \nu) - \Gamma^{T}(k\bfzeta))^{2} } \\
%     &= \argmin_{\Gamma \in \mathbb{R}^{d}} \EE[\epsilon \sim G, \nu \sim F, \bfzeta \sim R^{d}] { (\tilde{\ell}(\bfbeta + k\bfzeta, s, \nu, \epsilon ) - \Gamma^{T}(k\bfzeta))^{2}} \\
% \end{align*}

% As a result, we can apply Lemma \ref{lemm:linear_beta} to conclude that $\Gamma^{k}_{\ell, \bfbeta}(\bfbeta, s)$ limits to $\frac{\partial L}{\partial \bfbeta}(\bfbeta, s)$ as $k \rightarrow 0.$
% Since $\tau^{k}_{\text{ME}}(\bfbeta) = \Gamma^{k}_{\ell, \bfbeta}(\bfbeta, s(\bfbeta))$, we have that $\tau^{k}_{\text{ME}}(\bfbeta) \rightarrow \frac{\partial L}{\partial \bfbeta}(\bfbeta, s(\bfbeta)) = \tau_{\text{ME}}(\bfbeta)$ as $k \rightarrow 0.$



% First, we approximate $\frac{\partial s}{\partial \bfbeta}$ by estimating the partial MErivatives that appear in the right siME of \eqref{eq:ds_db}.

% Without loss of generality, for any one-dimensional parameter $\theta$, we show how to estimate $\frac{\partial P_{\bfbeta, s}(r)}{\partial \bfbeta}$ and $\frac{\partial P_{\bfbeta, s}(r)}{\partial \theta}$. Let us define a function $\Pi(\bfbeta, s)$ as follows
% \[ \Pi(\bfbeta, s; r) = 1 - P_{\bfbeta, s}(r).  \]
% Note that
% \[\frac{\partial P_{\bfbeta, s}(r)}{\partial \bfbeta} = -\frac{\partial \Pi}{\partial \bfbeta}(\bfbeta, s; r) \text{ and } \frac{\partial P_{\bfbeta, s}(r)}{\partial s} = -\frac{\partial \Pi}{\partial s}(\bfbeta, s; r).\]
% We can also define $\tilde{\pi}(\bfbeta, s, \nu, \epsilon; r)$ as follows
% \[\tilde{\pi}(\bfbeta, s, \nu, \epsilon; r) &= \pi_{\epsilon}(\bfg(\bfbeta, s, \nu); \bfbeta, r).\]
% We observe that
% \[\Pi(\bfbeta, s; r) = \EE[\epsilon \sim G, \nu \sim F]{\tilde{\pi}(\bfbeta,s, \nu, \epsilon; r) }.\]


% We note that $\Pi(\bfbeta, s; r)$ has the form required by the hypotheses of Lemma \ref{lemm:linear_beta}. In addition, we have that
% \begin{align*}
% \Gamma_{\pi, \bfbeta}^{k}(\bfbeta, s, r) &= \argmin_{\Gamma \in \mathbb{R}^{d}} \EE[\epsilon \sim G, \nu \sim F, \bfzeta \sim R^{d}] {( \pi_{\epsilon}(g(\bfbeta + k \bfzeta, s, \nu); \bfbeta + k\bfzeta, r) - \Gamma^{T}(k\bfzeta))^{2} }, \\
% &=  \argmin_{\Gamma \in \mathbb{R}^{d}} \EE[\epsilon \sim G, \nu \sim F, \bfzeta \sim R^{d}]{(\tilde{\pi}(\bfbeta + k\bfzeta,s, \nu, \epsilon; r) - \Gamma^{T}(k\bfzeta))^{2} }. \\
% \end{align*}

% Similarly, we have that $\Pi(\bfbeta, s; r)$ has the form required by Lemma \ref{lemm:linear_s}, and 

% \begin{align*}
% \Gamma_{\pi, s}^{k}(\bfbeta, s, r) &= \argmin_{\Gamma \in \mathbb{R}^{d}} \EE[\epsilon \sim G, \nu \sim F, \zeta \sim R] {(\pi_{\epsilon}(g(\bfbeta, s + k \zeta, \nu); \bfbeta, r) - \Gamma(k\zeta))^{2} } \\
% &= \argmin_{\Gamma \in \mathbb{R}^{d}} \EE[\epsilon \sim G, \nu \sim F, \zeta \sim R]{(\tilde{\pi}(\bfbeta,s + k \zeta, \nu, \epsilon; r) - \Gamma(k\zeta))^{2} }. \\
% \end{align*}

% Applying Lemma \ref{lemm:linear_beta} and Lemma \ref{lemm:linear_s} respectively yields \[\Gamma^{k}_{\pi, \bfbeta}(\bfbeta, s, r) \rightarrow \frac{\partial \Pi}{\partial \bfbeta}(\bfbeta, s; r) \quad \text{ and } \quad  \Gamma^{k}_{\pi, s}(\bfbeta, s, r) \rightarrow \frac{\partial \Pi}{\partial s}(\bfbeta, s; r)\] as $k \rightarrow 0.$


% We can apply the above results to compute $\frac{\partial s}{\partial \bfbeta}$ as follows
% \[-\Gamma^{k}_{\pi, \bfbeta}(\bfbeta, s(\bfbeta), r) \rightarrow \frac{\partial P_{\bfbeta, s(\bfbeta)}(r)}{\partial \bfbeta} \quad \text{ and } \quad  -\Gamma^{k}_{\pi, s}(\bfbeta, s(\bfbeta), r) \rightarrow \frac{ \partial P_{\bfbeta, s(\bfbeta)}(r)}{\partial s}\] as $k \rightarrow 0.$
% Thus, if we let $r= s(\bfbeta)$, we have that
% \begin{align*} \lim_{k_{1}, k_{2} \rightarrow 0} \frac{1}{p_{\bfbeta, s(\bfbeta)}(r) - \Gamma_{\pi, s}^{k_{2}}(\bfbeta, s(\bfbeta), r) }\cdot  \Gamma_{\pi, \bfbeta}^{k_{1}}(\bfbeta, s(\bfbeta), r)  &= \frac{1}{p_{\bfbeta, s(\bfbeta)}(r) - \frac{\partial \Pi}{\partial s}(\bfbeta, s(\bfbeta); r) } \cdot \frac{\partial \Pi}{\partial \bfbeta}(\bfbeta, s(\bfbeta); r) \\
% &= - \frac{1}{p_{\bfbeta, s(\bfbeta)}(r) + \frac{\partial P_{\bfbeta, s(\bfbeta)}(r)}{\partial s}} \cdot \frac{\partial P_{\bfbeta, s(\bfbeta)}(r)}{\partial \bfbeta } \\
% &= - \frac{1}{p_{\bfbeta, s(\bfbeta)}(s(\bfbeta)) + \frac{\partial P_{\bfbeta, s}(s(\bfbeta))}{\partial s}} \cdot \frac{\partial P_{\bfbeta, s}(s(\bfbeta))}{\partial \bfbeta } \\
% &= \frac{\partial s}{\partial \bfbeta}(\bfbeta)\\
% \end{align*}

% The last line follows from Lemma \ref{lemm:ds_dbeta}.

% We have that
% \[ \pi(r; \bfbeta, s) = \EE[\epsilon \sim G, \nu \sim F]{\mathbb{I}(\bfbeta^{T} \bfg(\bfbeta, s, \nu) + \epsilon > r)}.\]

% We note that $\pi$ has the form required by the hypotheses of Lemma \ref{lemm:linear_beta} and Lemma \ref{lemm:linear_s}. From Lemma \ref{lemm:linear_beta}, we have that $\Gamma^{k}_{\pi, \bfbeta} = \frac{\partial \pi }{\partial \bfbeta}$ as $k \rightarrow 0$ and from Lemma \ref{lemm:linear_s}, we have that $\Gamma^{k}_{\pi, s} =  \frac{\partial \pi }{\partial s} $ as $k \rightarrow 0.$ 

% Let $s^{*}=s(\bfbeta)$, the unique fixed point induced by the model $\bfbeta$. We have that
% \begin{align*}
%     \hat{\tau}_{\text{ME}, n}^{t}(\bfbeta) &=\hat{\Gamma}_{\ell, \bfbeta}(\bfbeta, \hat{s}^{t_{n}}_{n}, \hat{q}_{n}) \\
%     &= \hat{\Gamma}_{\ell, \bfbeta}(\bfbeta, s^{*}, s^{*}) + o_{p}(1) \\
%     &\xrightarrow{p} \frac{\partial L}{\partial \bfbeta}(\bfbeta, s^{*})\\
%     &= \tau_{\text{ME}} 
% \end{align*}
% The second line follows from  Corollary \ref{coro:convergence_in_prob_threshold}, which gives that $\hat{s}^{t_{n}}_{n} \xrightarrow{p} s^{*}.$ We also have that $\hat{q}_{n} \xrightarrow{p} s^{*}$ because the size of the perturbations limits to zero, the perceived threshold limits to $s^{*}$, so the realized empirical quantile limits to the realized population quantile, which is $s^{*}$. The third line holds because by Lemma \ref{lemm:gradient_estimators_converge} we have that $L(\bfbeta, s)$ satisfies the conditions of Lemma \ref{lemm:linear_beta}, so we have that our gradient estimator converges in probability to the true gradient.

% \begin{align*}
%     \hat{\Gamma}_{\ell, s}(\bfbeta, \hat{s}^{t_{n}}_{n}, q(\tilde{P}^{n}_{\bfbeta, s}) ) &= \hat{\Gamma}_{\ell, s}(\bfbeta, s^{*}, s^{*}) + o_{p}(1) \\
%     &\xrightarrow{p} \frac{\partial L}{\partial s}(\bfbeta, s^{*}).
% \end{align*}
% The first line follows from  Corollary \ref{coro:convergence_in_prob_threshold}, which gives that $\hat{s}^{t_{n}}_{n} \xrightarrow{p} s^{*}.$ We also have that $\hat{q}_{n} \xrightarrow{p} s^{*}$ because the size of the perturbations limits to zero, the perceived threshold limits to $s^{*}$, so the realized empirical quantile limits to the realized population quantile, which is $s^{*}$. The second line holds because by Lemma \ref{lemm:gradient_estimators_converge} we have that $L(\bfbeta, s)$ satisfies the conditions of Lemma \ref{lemm:linear_s}, so we have that our gradient estimator of $\frac{\partial L}{\partial s}$ converges in probability. 


% The proof consists of two parts, proving that the first term of the estimator in \eqref{eq:ie_estimator} converges in probability to $\frac{\partial L}{\partial s}(\bfbeta, s^{*})$ and proving that the second term of the estimator converges in probability $\frac{\partial s}{\partial \bfbeta}(\bfbeta)$. We state a technical lemma that will be used in the second part of the proof.

% We show that first term on the right of \eqref{eq:ie_estimator} converges in probability to $\frac{\partial L}{\partial s}(\bfbeta, s^{*})$.


% Now, we realize that
% \begin{align*}
%     |\hat{\Gamma}^{n}_{\ell, s}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}})) - \frac{\partial L}{\partial s}(\bfbeta, s^{*}, s^{*})| \leq&  |\hat{\Gamma}^{n}_{\ell, s}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}})) - \hat{\Gamma}^{n}_{\ell, s}(\bfbeta, s^{*} , s^{*})| \\
%     &+ ||.
% \end{align*}

% The first term on the right side converges in probability by \eqref{eq:convergence_in_prob_emp_gradient}. The second term on the right side converges in probability by Lemma \ref{lemm:linear_s}. 

%In \eqref{eq:ds_db_1}, we apply Slutsky's Theorem given Equations \ref{eq:dpi_ds}, \ref{eq:dpi_ds}, which gives that $\hat{s}^{t_{n}}_{n} \xrightarrow{p} s^{*}$. In \eqref{eq:ds_db_2}, we note that the empirical density function converges in probability to the population density function, so $p^{n}_{\bfbeta, s}(r) \xrightarrow{p} p_{\bfbeta, s}(r)$ for any choice of $\bfbeta, s, r.$ In \eqref{eq:ds_db_3}, we have that our gradient estimates of $\Pi(\bfbeta, s^{*}; s^{*})$ converge because by Lemma \ref{lemm:gradient_estimators_converge} $\Pi(\bfbeta, s; r)$ satisfies the conditions of Lemma \ref{lemm:linear_beta} and Lemma \ref{lemm:linear_s}. In \eqref{eq:ds_db_4}, we apply Lemma \ref{lemm:ds_dbeta}. Thus, we have that
% \begin{equation}
%     \label{eq:ds_db_convergence}
%         \frac{\hat{\Gamma}_{\pi, \bfbeta}(\bfbeta, \hat{s}^{t_{n}}_{n}; \hat{s}^{t_{n}}_{n})}{p^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}}(\hat{s}^{t_{n}}_{n}) - \hat{\Gamma}_{\pi, s}(\bfbeta, \hat{s}^{t_{n}}_{n}; \hat{s}^{t_{n}}_{n}) } \xrightarrow{p} \frac{\partial s}{\partial \bfbeta}(\bfbeta). \\
% \end{equation}


% \begin{lemm}
% \label{lemm:linear_r}
% Let $H$ denote the joint distribution over $\nu$ and $\epsilon.$ Let $Y(\bfbeta, s, r): \mathbb{R}^{d} \times \mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}$ be a differentiable function of the form \[Y(\bfbeta, s, r) = \EE[ (\nu, \epsilon) \sim H]{ y(\bfbeta, s, r, \nu, \epsilon)},\]
% where $y(\bfbeta, s, r, \cdot, \cdot, \cdot)$ is 
% \begin{enumerate}
%     \item Almost surely continuous in the sense that for each fixed $(s, r)$, the set $\{ (\nu, \epsilon) : \lim_{(s', r') \rightarrow (s, r)}  y(\bfbeta, s, r, \nu, \epsilon) \}$ has probability 1 $(dH)$ \\
%     \item Dominated, meaning that $|y(\bfbeta, s, r, \nu, \epsilon)| \leq a(\nu, \epsilon)$ where $b$ is integrable with respect to $H$.
% \end{enumerate}
% Let $b_{n}= bn^{-k}$ for $0< k < 0.5$ and $b > 0.$ Let $\mathbf{Z} \in \mathbb{R}^{n \times 1}$ be a matrix of perturbations, where the $i$-th row corresponds to $b_{n}\zeta_{i}$, where $\zeta_{i} \in R^{d}$, a Rademacher random variable. 
% Suppose that we have a vector of $n$ samples, $\mathbf{y} \in \mathbb{R}^{n}$, where \[\mathbf{y}_{i} = y(\bfbeta, s, r + b_{n}\zeta_{i}, \bfeta_{i}, \bfgamma_{i}, \epsilon_{i}).\]
% Let $\hat{\Gamma}^{n}(\bfbeta, s, r)$ the regression coefficient that is obtained by running OLS of $\mathbf{y}$ on $\mathbf{Z}.$ We have pointwise convergence in probability
% \[ \hat{\Gamma}^{n}(\bfbeta, s, r) \xrightarrow{p} \frac{\partial Y}{\partial r}(\bfbeta, s, r).\]

% In addition, for $\mathcal{S}$ compact, we have uniform convergence in probability
% \[ \sup_{(s,r) \in \mathcal{S} \times \mathcal{S}} \Big|\hat{\Gamma}^{n}(\bfbeta, s, r) - \frac{\partial Y}{\partial r}(\bfbeta, s, r)\Big| \xrightarrow{p} 0. \]
% \end{lemm}


% In the second part of the proof, we show that the gradient estimator converges to the true gradient uniformly in $(s,r).$
% For simplicity, for the remainder of the proof use the following abbreviations 
% \begin{align*}
%     \mathbf{z}&:= (\nu, \epsilon) \\
%     \pmb{\theta} &:= (s, r) \\
%     \Theta &: \mathcal{S} \times \mathcal{S}\\
%     y(\bfbeta, \pmb{\theta}, \mathbf{z}) &:= y(\bfbeta, s, r, \nu, \epsilon)\\
%     Y(\bfbeta, \pmb{\theta}) &:= Y(\bfbeta, s, r)\\ 
%     a(\mathbf{z}) &:= a(\nu, \epsilon)\\
%     \hat{\Gamma}_{n}(\bfbeta, s, r) &:= \hat{\Gamma}_{n}(\bfbeta, \bftheta). 
% \end{align*}
% Let $\epsilon> 0.$ We define 
% \begin{align*}
%     v(\mathbf{z}, \bfbeta, \bftheta, d) &=  \sup_{|\bftheta'- \bftheta| \leq d} |y(\bfbeta, \bftheta', \mathbf{z}) - y(\bfbeta, \bftheta, \bfz)|.
% \end{align*}
% By the almost sure continuity of $y$, we have that for fixed $\bftheta$
% \[ P\Big(\lim_{d \rightarrow 0} v(\mathbf{z}, \bfbeta, \bftheta, d) = 0\Big) = 1.\] Furthermore, we have that
% \begin{align*} P\Big( \lim_{d \rightarrow 0 } v(\bfz, \bfbeta + d \mathbf{e}_{j} , \bftheta, d) = 0\Big) &= 1 \\
% P\Big( \lim_{d \rightarrow 0 } v(\bfz, \bfbeta - d \mathbf{e}_{j} , \bftheta, d) = 0\Big) &= 1.
% \end{align*}
% In addition, we have that
% \begin{align*}
%     v(\bfbeta + d\mathbf{e}_{j}, \mathbf{z}, \bftheta, d) &\leq \sup_{\bfbeta \in \mathcal{B}} \sup_{|\bftheta' - \bftheta| \leq d} |y(\bfbeta - d\mathbf{e}_{j}, \bftheta', \mathbf{z})| + \sup_{\bfbeta \in \mathcal{B}} \sup_{|\bftheta' - \bftheta| \leq d} |y(\bfbeta + d\mathbf{e}_{j}, \bftheta, \bfz)| \\
%     &\leq a(\mathbf{z}) + a(\bfz) \\
%     &\leq 2a(\bfz),
% \end{align*}
% and $a(\mathbf{z})$ is integrable with respect to $H$, so by the Dominated Convergence Theorem we can say that $\EE[\mathbf{z}\sim H]{v(\bfbeta + d \mathbf{e}_{j}, \mathbf{z},\pmb{\theta}, d)}\leq \epsilon$ whenever $d \leq \delta_{1}^{+}(\bftheta, j),$ and $\EE[\mathbf{z}\sim H]{v(\bfbeta - d \mathbf{e}_{j}, \mathbf{z},\pmb{\theta}, d)}\leq \epsilon$ whenever $d \leq \delta_{1}^{-}(\bftheta, j).$ Let $\delta_{1}(\bftheta)$ be the minimum of all $\delta^{+}(\bftheta, j)$ and $\delta^{-}(\bftheta, j)$ for $j=1, 2, \dots d$.
% For $n$ large enough that $b_{n}$ is less than $\delta_{1}(\bftheta)$, we have that $\EE[\mathbf{z}\sim H]{v(\bfbeta + b_{n} \mathbf{e}_{j}, \mathbf{z},\pmb{\theta}, d)}\leq \epsilon$ for all $j$.

% In addition, we note that $\frac{\partial Y}{\partial \bfbeta}$ is a continuous function in $\bftheta$, so there exists $\delta_{2}(\bftheta)$ such that if $|\bftheta - \bftheta'| < \delta_{2}(\bftheta)$, then $|\frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta) - \frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta')| < \epsilon$. Let $\delta(\bftheta) = \min(\delta_{1}(\bftheta), \delta_{2}(\bftheta)).$

% Let $B(\bftheta)$ be an open ball of radius $\delta(\bftheta)$ about $\bftheta$. We note that $\mathcal{O} =\{ B(\bftheta) \}_{\bftheta \in \Theta}$ forms an open cover of $\Theta.$ By compactness of $\Theta$, there exists a finite subcover $\mathcal{O}' = \{ B(\bftheta_{k})\}_{k=1}^{K}$. Let
% $d_{k} = \delta(\bftheta_{k})$ and let $n_{k}$ be the smallest $n$ such that $b_{n} \leq d_{k},$ then for any $n \geq n_{k}$
% \begin{align}
% \EE{v(\bfbeta + b_{n}\mathbf{e}_{j}, \mathbf{z}, \bftheta_{k}, d_{k})} &\leq \epsilon \label{eq:bound_expected_v1}\\
% \EE{v(\bfbeta - b_{n}\mathbf{e}_{j}, \mathbf{z}, \bftheta_{k}, d_{k})} &\leq \epsilon.\label{eq:bound_expected_v2}
% \end{align}

% We proceed with the main argument of the proof. Let $\bftheta \in \Theta$. Then $\bftheta \in B(\bftheta_{k})$ for some $\bftheta_{k}$ such that $B(\bftheta_{k}) \in \mathcal{O}'.$ We see that
% \begin{align}
% \Big|\hat{\Gamma}^{n}(\bfbeta, \bftheta) - \frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta)\Big| 
% \leq& \Big| \hat{\Gamma}^{n}(\bfbeta, \bftheta) - \hat{\Gamma}^{n}(\bfbeta, \bftheta_{k}) \Big| + \Big| \hat{\Gamma}^{n}(\bfbeta, \bftheta_{k}) -  \frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta_{k}) \Big| \label{eq:bound_grad1}\\
% &+ \Big| \frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta_{k}) - \frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta) \Big| \label{eq:bound_grad2}
% \end{align}

% From \eqref{eq:ols_decomp}, we realize that we can rewrite $\hat{\Gamma}^{n}(\bfbeta, \bftheta)$ as follows
% \[ \hat{\Gamma}^{n}(\bfbeta, \bftheta) = (\mathbf{S}_{zz}^{n}^{n})^{-1}\mathbf{s}_{zy}^{n}(\bfbeta, \bftheta).\] We note that $\mathbf{y}$ is a function of $\bfbeta, \bftheta$, and $\mathbf{s}_{zy}^{n}$ is a function of $\mathbf{y}$. Meanwhile, $(\mathbf{S}_{zz}^{n}^{n})^{-1}$ is fixed for all choices of $\bftheta.$ We focus on the first term on the right side of \eqref{eq:bound_grad1}
% \begin{align}
%     \Big| \hat{\Gamma}^{n}(\bfbeta, \bftheta) - \hat{\Gamma}^{n}(\bfbeta, \bftheta_{k}) \Big| &= \Big|(\mathbf{S}_{zz}^{n}^{n})^{-1} \mathbf{s}_{zy}^{n}(\bftheta)  - (\mathbf{S}_{zz}^{n}^{n})^{-1} \mathbf{s}_{zy}^{n}(\bftheta_{k})\Big| \\
%     &\leq ||(\mathbf{S}_{zz}^{n}^{n})^{-1}||_{\text{op}} |\mathbf{s}_{zy}^{n}(\bftheta) - \mathbf{s}_{zy}^{n}(\bftheta_{k}) | \\
%     &\leq  ||(\mathbf{S}_{zz}^{n}^{n})^{-1}||_{\text{op}} \cdot \frac{1}{b_{n}} \cdot\Big| \frac{1}{n} \sum_{i=1}^{n} \bfzeta_{i} (\mathbf{y}_{i}(\bftheta) - \mathbf{y}_{i}(\bftheta_{k}) \Big|. \label{eq:emp_grad_final_bound}
% \end{align}

% We focus on the $j$-the entry of the last term on the right side of the above equation.

% \begin{align*}
%     \Big| \frac{1}{n} \sum_{i=1}^{n} \bfzeta_{i, j} (\mathbf{y}_{i}(\bftheta) - \mathbf{y}_{i}(\bftheta_{k}) \Big| =& \Big| \frac{1}{n} \Big(\sum_{i: \bfzeta_{i, j} = 1} y(\bfbeta + b_{n}\mathbf{e}_{j}, \bftheta, \bfz_{i}) - y(\bfbeta + b_{n}\mathbf{e}_{j}, \bftheta_{k}, \bfz_{i})  \\
%     &- \sum_{i: \bfzeta_{i, j} = -1} y(\bfbeta - b_{n}\mathbf{e}_{j}, \bftheta, \bfz_{i}) - y(\bfbeta - b_{n}\mathbf{e}_{j}, \bftheta_{k}, \bfz_{i}) \Big) \Big| \\
%     \leq&  \frac{1}{n} \Big(\sum_{i: \bfzeta_{i, j} = 1} |y(\bfbeta + b_{n}\mathbf{e}_{j}, \bftheta, \bfz_{i}) - y(\bfbeta + b_{n}\mathbf{e}_{j}, \bftheta_{k}, \bfz_{i})  \\
%     &+ \sum_{i: \bfzeta_{i, j} = -1} |y(\bfbeta - b_{n}\mathbf{e}_{j}, \bftheta, \bfz_{i}) - y(\bfbeta - b_{n}\mathbf{e}_{j}, \bftheta_{k}, \bfz_{i})| \Big) \\
%     \leq& \Big| \frac{1}{n} \sum_{i: \bfzeta_{i, j} = 1} v(\bfz_{i}, \bftheta_{k}, \bfbeta + b_{n}\mathbf{e}_{j}, d_{k})| +  \Big| \frac{1}{n} \sum_{i: \bfzeta_{i, j} = -1} v(\bfz_{i}, \bftheta_{k}, \bfbeta - b_{n}\mathbf{e}_{j}, d_{k}) \Big| \\
% \end{align*}

% For fixed $b_{n},$ by the Weak Law of Large Numbers, we have that \begin{align*}
% \frac{1}{n} \sum_{i=1}^{n} v(\mathbf{z}_{i}, \bfbeta + \mathbf{e}_{j}, \bftheta_{k}, d_{k}) &\xrightarrow{p} \EE{v(\bfbeta + b_{n}\mathbf{e}_{j}, \mathbf{z}, \bftheta_{k}, d_{k})}\\
% \frac{1}{n} \sum_{i=1}^{n} v(\mathbf{z}_{i}, \bfbeta - \mathbf{e}_{j}, \bftheta_{k}, d_{k}) &\xrightarrow{p} \EE{v(\bfbeta + b_{n}\mathbf{e}_{j}, \mathbf{z}, \bftheta_{k}, d_{k})},
% \end{align*}
% and for large enough $n$ we have that the expectations on the right side are less than $\epsilon$ from Equations \ref{eq:bound_expected_v1} and \ref{eq:bound_expected_v2}. In addition, we recall that Equations \ref{eq:converge_to_half1} and \ref{eq:converge_to_half2} holds. Applying Slutsky's Theorem, we conclude that for any fixed $j$, \[\Big| \frac{1}{n} \sum_{i=1}^{n} \mathbf{w}eta_{i, j} (\mathbf{y}_{i}(\bftheta) - \mathbf{y}_{i}(\bftheta_{k}) \Big| = o_{p}(1).\] Similarly, when we consider all $d$ dimensions, we must have \[\Big| \frac{1}{n} \sum_{i=1}^{n} \bfzeta_{i} (\mathbf{y}_{i}(\bftheta) - \mathbf{y}_{i}(\bftheta_{k}) \Big| = o_{p}(1).\]
% Now, we can return to analyzing $\Big| \hat{\Gamma}^{n}(\bfbeta, \bftheta) - \hat{\Gamma}^{n}(\bfbeta, \bftheta_{k}) \Big|$ in \eqref{eq:emp_grad_final_bound}. From \eqref{eq:s_zz}, we note that $\mathbf{S}_{zz}^{n}^{n} \xrightarrow{p} I_{d}$, so by Slutsky's Theorem and the Continuous Mapping Theorem $||(\mathbf{S}_{zz}^{n}^{n})^{-1}||_{\text{op}} \xrightarrow{p} 1.$ Furthermore, $\frac{1}{b_{n}} \rightarrow 0.$ As a result, we conclude that \[\Big| \hat{\Gamma}^{n}(\bfbeta, \bftheta) - \hat{\Gamma}^{n}(\bfbeta, \bftheta_{k}) \Big| = o_{p}(1).\]

% By our pointwise convergence result in the first part of the proof, the second term on the right side of \eqref{eq:bound_grad1} is also $o_{p}(1)$. Finally, the term in \eqref{eq:bound_grad2} is guaranteed to be less than or equal to $\epsilon$ due to our construction of the cover. Since the argument above holds for any $\bftheta \in \Theta$, we have that
% \[ \sup_{\bftheta \in \Theta} \Big|\hat{\Gamma}^{n}(\bfbeta, \bftheta) - \frac{\partial Y}{\partial \bfbeta}(\bfbeta, \bftheta')\Big| \xrightarrow{p} 0.\]
% Removing our abbreviations, this gives our desired claim
% \[ \sup_{ (s, r) \in \mathcal{S} \times \mathcal{S}} \Big|\hat{\Gamma}^{n}(\bfbeta, s, r) - \frac{\partial Y}{\partial \bfbeta}(\bfbeta, s, r)\Big| \xrightarrow{p} 0. \]


% \begin{subsection}{Proof of Theorem \ref{theo:direct_effect}}
% We consider the collection of stochastic processes $\{\hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta, s , r)\}$ indexed by $(s, r) \in \mathcal{S} \times \mathcal{S}$. By Lemma \ref{lemm:gradient_estimators_converge}, the function $L(\bfbeta, s)$ can be rewritten in a form that satisfies the conditions of Lemma \ref{lemm:linear_beta}. This gives us that $\hat{\Gamma}^{n}_{\ell, \bfbeta}$ converges in probability pointwise to $\frac{\partial L}{\partial \bfbeta}$ and is stochastically equicontinuous. In particular, $\{\hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta, s, r)\}$ is stochastically equicontinuous at index $(s^{*}, s^{*}) \in \mathcal{S} \times \mathcal{S}.$

% We recall that by Corollary \ref{coro:convergence_in_prob_threshold} gives that
% \[ \hat{s}^{t_{n}}_{n} \xrightarrow{p} s^{*}\]
% and Lemma \ref{lemm:quantile_perturbed_stoch_process} gives that
% \[ q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b_{n}}) \xrightarrow{p} s^{*},\]
% so we can apply Lemma \ref{lemm:stochastic_equicontinuity_convergence_in_prob} to conclude that
% \begin{equation} 
% \label{eq:convergence_in_prob_emp_gradient}
% \hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b_{n}}))  - \hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta, s^{*} , s^{*}) \xrightarrow{p} 0.\end{equation}
% Now, we realize that
% \begin{align*}
%     |\hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}})) - \frac{\partial L}{\partial \bfbeta}(\bfbeta, s^{*})| \leq&  |\hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}})) - \hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta, s^{*} , s^{*})| \\
%     &+ |\hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta, s^{*} , s^{*}) - \frac{\partial L}{\partial \bfbeta}(\bfbeta, s^{*})|.
% \end{align*}

% The first term on the right side converges in probability by \eqref{eq:convergence_in_prob_emp_gradient}. The second term on the right side converges in probability by Lemma \ref{lemm:linear_beta}. Therefore, we have that 

% \[ \hat{\tau}_{\text{ME}, n}^{t} = \hat{\Gamma}^{n}_{\ell, \bfbeta}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}})) \xrightarrow{p} \frac{\partial L}{\partial \bfbeta}(\bfbeta, s^{*}) = \tau_{\text{ME}}.\]



% \end{subsection}


% \begin{lemm}
% \label{lemm:loss_deriv_pointwise_equicontinuity}
% Suppose Assumptions \ref{assumption:strong_convexity}, \ref{assumption:prob_second_deriv_bound}, \ref{assumption:cdf_noise_strictly_increasing}, \ref{assumption:br_interior}, and \ref{assumption:bounded_noise} hold. Let $b_{n}= bn^{-k}$ for $0< k < 0.5$ and $b > 0.$ Let $\mathbf{Z} \in \mathbb{R}^{n \times d}$ be a matrix of perturbations, where the $i$-th row corresponds to $b_{n}\bfzeta_{i}^{T}$, where $\bfzeta_{i} \in R^{d}$, a $d$-dimensional Rademacher random variable.
% Suppose we observe $P^{n}_{\bfbeta, s, b_{n}}$ and $\pmb{\ell} \in \mathbb{R}^{n}$ as defined in \eqref{eq:direct_effect_loss}.
% Let $\hat{\Gamma}^{n}(\bfbeta, s)$ the regression coefficient that is obtained by running OLS of $\pmb{\ell}$ on $\mathbf{Z}.$ We have pointwise convergence in probability 
% \[ \hat{\Gamma}^{n}(\bfbeta, s) \xrightarrow{p} \frac{\partial L}{\partial \bfbeta}(\bfbeta, s).\]
% In addition, we have uniform convergence in probability
% \[ \sup_{s \in \mathcal{S}} \Big|\hat{\Gamma}^{n}(\bfbeta, s) - \frac{\partial L}{\partial \bfbeta}(\bfbeta, s)\Big| \xrightarrow{p} 0. \]
% \end{lemm}

% \begin{lemm}
% \label{lemm:linear_beta}
% Let $H$ denote the joint distribution over $\nu$ and $\epsilon.$ Let $Y(\bfbeta, s): \mathbb{R}^{d} \times \mathbb{R} \rightarrow \mathbb{R}$ be a differentiable function of the form \[Y(\bfbeta, s) = \EE[ (\nu, \epsilon) \sim H]{ y(\bfbeta, s, \nu, \epsilon)},\]
% where $y$ is 
% \begin{enumerate}
%     \item Almost surely continuous in the sense that for each fixed $s$, the set $\{ (\nu, \epsilon) : \lim_{s' \rightarrow s}  y(\bfbeta, s, \nu, \epsilon) \}$ has probability 1 $(dH)$. \\
%     \item Dominated, meaning that $|y(\bfbeta, s, \nu, \epsilon)| \leq a(\nu, \epsilon)$ where $a$ is integrable with respect to $H$.
% \end{enumerate}

% \begin{lemm}
% \label{lemm:linear_s}
% Let $H$ denote the joint distribution over $\nu$ and $\epsilon.$ Let $Y(\bfbeta, s, r): \mathbb{R}^{d} \times \mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}$ be a differentiable function of the form \[Y(\bfbeta, s, r) = \EE[ (\nu, \epsilon) \sim H]{ y(\bfbeta, s, r, \nu, \epsilon)},\]
% where $y(\bfbeta, s, r, \cdot, \cdot, \cdot)$ is 
% \begin{enumerate}
%     \item Almost surely continuous in the sense that for each fixed $(s, r)$, the set $\{ (\nu, \epsilon) : \lim_{(s', r') \rightarrow (s, r)}  y(\bfbeta, s, r, \nu, \epsilon) \}$ has probability 1 $(dH)$. \\
%     \item Dominated, meaning that $|y(\bfbeta, s, r, \nu, \epsilon)| \leq a(\nu, \epsilon)$ where $b$ is integrable with respect to $H$.
% \end{enumerate}
% Let $b_{n}= bn^{-k}$ for $0< k < 0.5$ and $b > 0.$ Let $\mathbf{Z} \in \mathbb{R}^{n \times 1}$ be a matrix of perturbations, where the $i$-th row corresponds to $b_{n}\zeta_{i}$, where $\zeta_{i} \in R^{d}$, a Rademacher random variable. 
% Suppose that we have a vector of $n$ samples, $\mathbf{y} \in \mathbb{R}^{n}$, where \[\mathbf{y}_{i} = y(\bfbeta, s+ b_{n}\zeta_{i}, r, \bfeta_{i}, \bfgamma_{i}, \epsilon_{i}).\]
% Let $\hat{\Gamma}^{n}(\bfbeta, s, r)$ the regression coefficient that is obtained by running OLS of $\mathbf{y}$ on $\mathbf{Z}.$ We have pointwise convergence in probability
% \[ \hat{\Gamma}^{n}(\bfbeta, s, r) \xrightarrow{p} \frac{\partial Y}{\partial s}(\bfbeta, s, r).\]

% In addition, for $\mathcal{S}$ compact, we have uniform convergence in probability
% \[ \sup_{(s,r) \in \mathcal{S} \times \mathcal{S}} \Big|\hat{\Gamma}^{n}(\bfbeta, s, r) - \frac{\partial Y}{\partial s}(\bfbeta, s, r)\Big| \xrightarrow{p} 0. \]
% \end{lemm}

% \begin{lemm}
% \label{lemm:gradient_estimators_converge}
% Under Assumptions \ref{assumption:strong_convexity}, \ref{assumption:prob_second_deriv_bound}, \ref{assumption:cdf_noise_strictly_increasing}, and \ref{assumption:br_interior}, $L(\bfbeta, s)$ and $\Pi(\bfbeta, s; r)$ can be written in a form that satisfies the conditions on $Y(\bfbeta, s, r)$ in Lemmas \ref{lemm:linear_beta} \ref{lemm:linear_s}.
% \end{lemm}

% \begin{lemm}
% \label{lemm:quantile_perturbed_simple}
% Fix $\bfbeta \in \mathcal{B}$. Under the conditions of Theorem \ref{theo:emp_fpi_convergence}, \[q(P^{n}_{\bfbeta, s, b_{n}}) \xrightarrow{p} q(P_{\bfbeta, s}).\]
% \end{lemm}

%In the first step of the proof, we use the property of stochastic equicontinuity to show that our gradient estimators defined in Definition \ref{defi:indirect_effect_estimator} converge in probability to gradient estimators evaluated at the equilibrium threshold $s^{*}$. In the second step of the proof, we use the pointwise convergence in probability results from Lemmas \ref{lemm:linear_beta} and \ref{lemm:linear_s} to show that the gradient estimators evaluated at the equilibrium point $s^{*}$ converge in probability to the true gradients. 

% We proceed with the main proof. We consider the following collections of stochastic processes indexed by $(s, r) \in \mathcal{S} \times \mathcal{S}$
% \[\{\hat{\Gamma}^{n}_{\ell, s}(\bfbeta, s , r)\}, \quad \{\hat{\Gamma}^{n}_{\pi, s}(\bfbeta, s , r)\}, \quad \{\hat{\Gamma}^{n}_{\pi, \beta}(\bfbeta, s , r)\}.\]
% By Lemma \ref{lemm:gradient_estimators_converge}, the functions $L(\bfbeta, s)$ and $\Pi(\bfbeta, s; r)$ can be rewritten in a form that satisfies the conditions of Lemma \ref{lemm:linear_beta} and Lemma \ref{lemm:linear_s}. This gives us that the above processes are stochastically equicontinuous. In particular, they are stochastically equicontinuous at index $(s^{*}, s^{*}) \in \mathcal{S} \times \mathcal{S}.$ The stochastic equicontinuity property of the gradient estimators enables us to apply Lemma \ref{lemm:stochastic_equicontinuity_convergence_in_prob} as follows. We recall that
%  Corollary \ref{coro:convergence_in_prob_threshold} gives that
% \[ \hat{s}^{t_{n}}_{n} \xrightarrow{p} s^{*}\]
% and Lemma \ref{lemm:quantile_perturbed_stoch_process} gives that
% \[ q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b_{n}}) \xrightarrow{p} s^{*},\]
% so we can apply Lemma \ref{lemm:stochastic_equicontinuity_convergence_in_prob} to conclude that
% \begin{align*} 
% \hat{\Gamma}^{n}_{\ell, s}(\bfbeta,  \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b_{n}}))  - \hat{\Gamma}^{n}_{\ell, s}(\bfbeta, s^{*} , s^{*}) &\xrightarrow{p} 0, \\ %\label{eq:emp_dl_ds} \\
% \hat{\Gamma}^{n}_{\pi, s}(\bfbeta,  \hat{s}^{t_{n}}_{n}, \hat{s}^{t_{n}}_{n})  - \hat{\Gamma}^{n}_{\pi, s}(\bfbeta, s^{*} , s^{*}) &\xrightarrow{p} 0, \\ %\label{eq:emp_dpi_ds} \\
% \hat{\Gamma}^{n}_{\pi, \bfbeta}(\bfbeta,  \hat{s}^{t_{n}}_{n}, \hat{s}^{t_{n}}_{n})  - \hat{\Gamma}^{n}_{\pi, \bfbeta}(\bfbeta, s^{*} , s^{*}) &\xrightarrow{p} 0 \\ %\label{eq:emp_dpi_dbeta}.
% \end{align*}

% In the second part of the proof, we can use the pointwise convergence results from Lemma \ref{lemm:linear_beta} and Lemma \ref{lemm:linear_s} to see that
% \begin{align*}
%     \hat{\Gamma}^{n}_{\ell, s}(\bfbeta, s^{*} , s^{*}) &\xrightarrow{p} \frac{\partial L}{\partial s}(\bfbeta, s^{*}), \\
%     \hat{\Gamma}^{n}_{\pi, s}(\bfbeta, s^{*} , s^{*}) &\xrightarrow{p} \frac{\partial \Pi}{\partial s}(\bfbeta, s^{*}, s^{*}), \\
%     \hat{\Gamma}^{n}_{\pi, \bfbeta}(\bfbeta, s^{*} , s^{*}) &\xrightarrow{p} \frac{\partial \Pi}{\partial \bfbeta}(\bfbeta, s^{*}).
% \end{align*}


% Therefore, we have that 
% \begin{align} 
% \hat{\Gamma}^{n}_{\ell, s}(\bfbeta, \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}, b_{n}}_{n}})) &\xrightarrow{p} \frac{\partial L}{\partial s}(\bfbeta, s^{*}),  \\
% \hat{\Gamma}^{n}_{\pi, s}(\bfbeta,  \hat{s}^{t_{n}}_{n}, \hat{s}^{t_{n}}_{n}) &\xrightarrow{p} \frac{\partial \Pi}{\partial s}(\bfbeta, s^{*}; s^{*}),  \\
% \hat{\Gamma}^{n}_{\pi, \bfbeta}(\bfbeta,  \hat{s}^{t_{n}}_{n}, \hat{s}^{t_{n}}_{n}) &\xrightarrow{p} \frac{\partial \Pi}{\partial \bfbeta}(\bfbeta, s^{*}; s^{*}).  
% \end{align}

% \label{lemm:stoch_equi_quantile}
% Under the conditions of Theorem \ref{theo:emp_fpi_convergence}, we have that the collection of stochastic processes $\{q(P^{n}_{\bfbeta, s})\}$ indexed by $s \in \mathcal{S}$ is stochastically equicontinuous.
% \end{lemm}

    %=& \frac{1}{n} \Big(\sum_{i: \bfzeta_{i, j} = 1} \tilde{\ell}(\mathbf{w}_{i}, \bfbeta + b \mathbf{e}_{j}, \hat{s}^{t_{n}}_{n} + b\zeta_{i}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}, b}) - b\zeta_{i}) \\
    %&-\sum_{i: \bfzeta_{i, j} = -1}\tilde{\ell}(\mathbf{w}_{i}, \bfbeta - b \mathbf{e}_{j}, \hat{s}^{t_{n}}_{n} + b\zeta_{i}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}, b}) - b\zeta_{i}) \Big) \\
    %=&\frac{n_{1, j}}{n} \cdot \tilde{\ell}_{n_{1, j}}(\bfbeta + b \mathbf{e}_{j}, \hat{s}^{t_{n}}_{n} + b\zeta_{i}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b}) - b\zeta_{i}) \\
    %&- \frac{n_{2, j}}{n} \tilde{\ell}_{n_{2, j}}(\bfbeta - b \mathbf{e}_{j}, \hat{s}^{t_{n}}_{n} + b\zeta_{i}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b}) - b\zeta_{i}). \label{eq:s_zy_part1} 
    % \rightarrow& \frac{n_{1, j}}{n} \tilde{\ell}_{n_{1, j}}(\bfbeta + b \mathbf{e}_{j}, \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b})) \\
    % &- \frac{n_{2, j}}{n} \tilde{\ell}_{n_{2, j}}(\bfbeta - b \mathbf{e}_{j}, \hat{s}^{t_{n}}_{n}, q(P^{n}_{\bfbeta, \hat{s}^{t_{n}}_{n}, b})) 
    
    \begin{subsection}{Proof of Lemma \ref{lemm:truncation}}
\label{subsec:truncation}
Let $s(\bfbeta, b)$ be the unique fixed point of $q(P_{\bfbeta, s, b}).$
\[\hat{s}^{t+1}_{A, n} = q(P_{\bfbeta, \hat{s}^{t}_{A, n}, b}) \]
Let $q = q(P_{\bfbeta, \hat{s}^{t}_{B, n}, b}).$
\[\hat{s}^{t+1}_{B, n} = \begin{cases} -S & q < -S \\ q & -S \leq q \leq S \\ S & q > S \end{cases}.\]
\begin{align*}
    P(\hat{s}^{t}_{A, n} \neq \hat{s}^{t}_{B, n} \mid \hat{s}^{t-1}_{A, n} = \hat{s}^{t-1}_{B, n}) &= P(q(P_{\bfbeta, \hat{s}^{t-1}_{B, n}, b}) > S \mid \hat{s}^{t-1}_{A, n} = \hat{s}^{t-1}_{B, n}) \\
    &\indent+  P(q(P_{\bfbeta, \hat{s}^{t-1}_{B, n}, b}) < -S \mid \hat{s}^{t-1}_{A, n} = \hat{s}^{t-1}_{B, n}) \\
    &= P(q(P_{\bfbeta, \hat{s}^{t-1}_{A, n}, b}) > S \mid \hat{s}^{t-1}_{A, n} = \hat{s}^{t-1}_{B, n}) \\
    &\indent+  P(q(P_{\bfbeta, \hat{s}^{t-1}_{A, n}, b}) < -S \mid \hat{s}^{t-1}_{A, n} = \hat{s}^{t-1}_{B, n}) \\
    &= P(\hat{s}^{t}_{A, n} > S) + P(\hat{s}^{t}_{A, n} < -S) \\
    &\leq P(|\hat{s}^{t}_{A, n} - s^{*}| > \min(S - s^{*}, -S -s^{*})) \\
    % &\leq \delta.
\end{align*}
\end{subsection}
